Clustered Relational Thread-Modular Abstract Interpretation with Local Traces

We construct novel thread-modular analyses that track relational information for potentially overlapping clusters of global variables - given that they are protected by common mutexes. We provide a framework to systematically increase the precision of clustered relational analyses by splitting control locations based on abstractions of local traces. As one instance, we obtain an analysis of dynamic thread creation and joining. Interestingly, tracking less relational information for globals may result in higher precision. We consider the class of 2-decomposable domains that encompasses many weakly relational domains (e.g., Octagons). For these domains, we prove that maximal precision is attained already for clusters of globals of sizes at most 2.

==> correctness/max-relational-domain.tex <==
\section{Maximally relational domain}
\[
  \begin{array}{lll}
    \alpha_{\bar {R_S}}(t) &=& \{ \sigma \in ((\X \cup \G \cup \{\returnVar\})\to\V) \mid\\
    && \quad \forall x\in\X: \sigma\,x = t(x),\\
    && \quad \forall g \in\G: \MM[g]\cap L[t] \neq \emptyset \implies \sigma\,g=t(g) \}\\[1ex]

    \alpha_{\bar {R_M}, m}(t) &=& \{ \sigma \in ((\X \cup \G \cup \{\returnVar\})\to\V) \mid\\
    && \quad \forall g \in\G: m\in\MM\,[g] \implies \sigma\,g=t(g) \}\\[1ex]

    \alpha_{\bar {R_M}, i}(t) &=& \{ \sigma \in ((\X \cup \G \cup \{\returnVar\})\to\V) \mid\\
    && \quad \TLr\,t=((u,\sigma_0),\return x,\_)\\
    && \qquad \implies \sigma\,\returnVar =\sigma_0\,x \}
  \end{array}
\]
where $L[t]$ denotes the set of locks held by the ego-thread at the end of a local trace and $t(g)$ is extended to extract the value written
at the last write to $g$ appearing in the local trace, or $0$ if no such write exists.

Here $\sqcap$ and $\sqcup$ correspond to $\cap$ and $\cup$, and the restriction $\restr{}{W}$ is defined by
\[
    \begin{array}{lll}
        \restr{S}{W} &=& \bigcup_{\sigma\in S} \{ \sigma'\in ((\X \cup \G \cup \{\returnVar\})\to\V) \mid\\
        && \qquad\quad \forall w\in W \sigma'\,w = \sigma\,w \}
    \end{array}
\]

Most relational domains can be seen as further abstractions of a basic relational domain that collects sets of assignments from some set of
variables $V$ to values from some set $\V$, i.e. ($\R_B=2^{V\to\V})$. In such a domain, least upper bound $\sqcup$ and greatest lower bound
$\sqcap$ simply correspond to $\cup$ and $\cap$, and parallel assignment $\aSem{\{x \leftarrow e_1, y \leftarrow e_2\}}_{\R_B}$ is
simply defined element-wise.
We also require a restriction $\restr{}{W}$ to some subset $W \subseteq V$ that is defined by
\[
    \begin{array}{lll}
        \restr{S}{W} &=& \bigcup_{\sigma\in S} \{ \sigma'\in \R_B \mid \forall w\in W: \sigma'\,w = \sigma\,w \}
    \end{array}
\]
This corresponds to adding mappings with all possible combinations of values for all variable that are not in $W$, and thus amounts to forgetting
all information for those variables not in $W$.
% Relational Domains that provide all these operations (and typically also operations $\widen$ and $\narrow$ that are
% crucial for practical implementations) are, e.g., Octagons\cite{Mine01}, Polyhedra\cite{...}, or Linear Equalities\cite{...}.

Given that abstract values always have all possible combinations of values for some variables (no information on these is maintained), one can
efficiently represent them in an abstraction, by only explicitly representing those variables for which information is maintained.
This is the key to efficient implementations of abstractions of $\R_B$.
Given a set $Q \subseteq 2^V$ of (possibly overlapping) clusters that should be maintained, once can decompose an abstract value from $\R_B$ into a
set of abstract values from $2^{\R_B}$, where each element is obtained by restricting the original value to the corresponding cluster. The operations
are the simply applied per cluster.
To go back to values from $\R_B$ one can simply take the meet of all clusters. In general, going from $\R_B$ to $2^{\R_B}$ and back
looses some information. However, for some abstractions of $\R_B$, there may be clusterings (that do not contain $V$ as a cluster),
that still preserve all information. For example, provided that the \emph{closure} operation is applied before restriction in the
\emph{Octagon}\cite{Mine01} domain, this applies when considering all two-variable clusters.

